XNAS: Neural Architecture Search with Expert Advice

This paper introduces a novel optimization method for differential neural architecture search, based on the theory of prediction with expert advice. Its optimization criterion is well fitted for an architecture-selection, i.e., it minimizes the regret incurred by a sub-optimal selection of operations. Unlike previous search relaxations, that require hard pruning of architectures, our method is designed to dynamically wipe out inferior architectures and enhance superior ones. It achieves an optimal worst-case regret bound and suggests the use of multiple learning-rates, based on the amount of information carried by the backward gradients. Experiments show that our algorithm achieves a strong performance over several image classification datasets. Specifically, it obtains an error rate of 1.6% for CIFAR-10, 24% for ImageNet under mobile settings, and achieves state-of-the-art results on three additional datasets.

==> Methodology/wipeout_mechanism.tex <==
\label{sec:wipeout_mechanism}

==> advantages_of_the_proposed_method/advantages_of_the_proposed_method.tex <==
\subsection{The Recovery of Late Bloomers}
In this section we demonstrate how GD with softmax depresses initially weak operations as XNAS mitigates the effect.
We derive the corresponding update rules and explain the underlying functional structure.
\input{advantages_of_the_proposed_method/recovery_of_late_blommers.tex}

\subsubsection{A Deterministic Toy Example}
\input{advantages_of_the_proposed_method/deterministic_toy.tex}


\subsection{No Weight Decay}
\input{advantages_of_the_proposed_method/no_weight_decay.tex}

==> analysis_and_discussion/theoretical_analysis_no_rescale.tex <==
\label{sec:theoretical_analysis}
In this section we introduce the \emph{regret} as a performance measure for NAS algorithms, provide theoretical guarantees for XNAS with respect to this measure and to the promise of not wiping out the best expert. Proofs appear in \ref{subsec:proofs} for brevity. %of the supplementary material.
We also extract practical instructions from theory with regard to the choice of multiple learning rates. Finally we briefly discuss the equivalence of our reward to the one considered by the policy gradient approach applied to NAS.

\textbf{The Regret as a Performance Measure.} In classical learning theory, statistical properties of the underlying process may be estimated on the basis of stationarity assumptions over the sequence of past observations. Thus effective prediction rules can be derived from these estimates~\cite{cesa2006prediction}. NAS methods that alternately learn the architecture weights and train the network weights are highly non-stationary.
In PEA theory, no statistical assumptions are made as ``simplicity is a merit''~\cite{hazan2016introduction}, and worst-case bounds are derived for the forecaster's performance.

Denote the regret and the cumulative losses of the forecaster and of the $i$th expert at time $t$ by,
\begin{align}
\label{losses_and_regret}
\textrm{Regret}_t = L_t-\min_{i=1,\dots N}L_{t,i}   \quad ; \quad 
 L_t=\sum_{s=1}^{t}\ell_s(p_s) \quad ; \quad  L_{t,i} = \sum_{s=1}^t \ell_s(f_{i,s})
\end{align} 
respectively. The regret measures how much the forecaster regrets not following the advice of the best expert in hindsight. This criterion suits our setup as we optimize a mixture of experts and select the best one by the end of the process.
\\
\textbf{A Safe Wipeout.} In XNAS, experts with no chance of taking the lead by the end of the search are wiped-out along the process. In a worse-case setup, a single incorrect wipeout might result in a large regret, i.e. linear in the number of steps $T$. The following lemma assures that this cannot happen,
\begin{lemma}
\label{no_wipe}
In XNAS, The optimal expert in hindsight cannot be wiped-out. 
\end{lemma}

\textbf{Regret Bounds.} Our main theorem guarantees an upper bound for the regret, 
\begin{theorem}[XNAS Regret Bound]
\label{EGW_Optimality}
The regret of the XNAS algorithm \ref{alg:XNAS}, with $N$ experts and learning rate $\eta$, incurring a sequence of $T$ non-negative convex losses of $\mathcal{L}$-bounded rewards, satisfies,
% Under previous assumptions, XNAS regret satisfies,
\begin{align}\label{eq:regret_bound}
\mathrm{Regret}_T \leq \frac{\eta T \mathcal{L}^2}{2} +\frac{1}{\eta}\ln N
\end{align}
\end{theorem}
Choosing the minimizer $\eta^*$ of \eqref{eq:regret_bound} yields the following tight upper bound,
\begin{align}
\label{eq:eta_and_regret}
\eta^*=\frac{1}{\mathcal{L}}\sqrt{\frac{2\ln N}{T}} \quad ; \quad \mathrm{Regret}_T  \leq \mathcal{L}\sqrt{2T\ln N}
\end{align}
The regret upper bound of XNAS is tight, as the lower bound can be shown to be of $\Omega(\mathcal{L}\sqrt{T\ln{N}})$~\cite{haussler1995tight}. For comparison, under the same assumptions, the worst-case regret bound of gradient-descent is of $O(\mathcal{L}\sqrt{T N})$~\cite{hazan2016introduction}, while the one of ADAM is linear in $T$~\cite{reddi2019convergence}. 
An illustration of the relationship between the regret and the rate of correct expert selection is left to \ref{sec:stochastic_toy} of the supplementary material. XNAS is shown to achieve a better regret compared to other optimizers.  

\textbf{Multiple Learning Rates.} Equation \ref{eq:eta_and_regret} connects the optimal theoretical learning rate $\eta^*$ with the number of steps $T$, which is also the number of gradient feedbacks received by the experts. Since forecasters weights are being replicated among different cells, the number of feedbacks is different for normal and reduction cells. explicitly, $T_c = \mathbf{D} \times \mathcal{E} \times \mathcal{R}_c$, where $\mathbf{D},\mathcal{E},\mathcal{R}_c$ are the validation set size, the number of epochs and the number of replications for cell type $c$ respectively. We adopt the use of multiple learning rates $\eta^*_c$ in our experiments. 
\\
\textbf{The Connection to Policy Gradient.} We conclude this section by pointing out an interesting connection between \emph{policy gradient} in NAS \cite{zoph2016neural} and PEA theory. We refer to the PEA based reward term in line~\ref{update_reward} of algorithm \ref{alg:XNAS}. This reward has been shown by \cite{snas} to be the same effective reward of a policy gradient method applied to the common NAS optimization criterion~\cite{zoph2016neural, NASNET,ENAS}. More precisely, consider the case where instead of mixing the experts predictions, the forecaster is to sample a single expert at each step with probability $u_{t,i}$. Then the effective reward associated with the policy gradient is exactly the derived PEA reward, $R_{t,i}=-\nabla_{p_t}\ell_t (p_t)\cdot f_{t,i}$.

==> experiments/tables_3.tex <==
\begin{table}[tb]
   \begin{minipage}[b]{.45\linewidth}
       \centering
            \begin{tabular}{|l|c|c|c|}
             \hline
            \vtop{\hbox{\strut \textbf{CIFAR-10}}\hbox{\strut Architecture}}
                & \multicolumn{1}{|p{0.75cm}}{\centering Test \\error}
                & \multicolumn{1}{|p{0.9cm}}{\centering Params\\(M) }
                & \multicolumn{1}{|p{0.8cm}|}{\centering Search\\cost}\\
                \hline
                AutoAugment \cite{cubuk2018autoaugment}  & $1.48$  & $26$  & $20$ \\    
                \hline
                NAONet-WS \cite{NAO} & $3.53$ & $2.5$ & $0.3$ \\   			
                PNAS \cite{PNAS} & $3.41$  & $3.2$  & $150$ \\  			
                Amoeba-A \cite{Real18Regularized}     & $3.34$  & $3.2$  & $3150$ \\
                DSO-NAS \cite{DSO} & $2.95$ & $3$ & $1$ \\
                DARTS(1nd) \cite{liu2018darts}      & $2.94$       & $2.9$  & $0.4$ \\
                ENAS \cite{ENAS} & $2.89$  & $4.6$  & $0.5$ \\
                SNAS \cite{snas} & $2.85$ & $2.8$ & $1.5$ \\
                % PARSEC \cite{casale2019probabilistic} & $2.81$ & $3.7$ & $1$ \\
                DARTS(2nd) \cite{liu2018darts} & $2.67$  & $3.4$  & $1$ \\
                NASNet-A \cite{NASNET}  & $2.65$      & $3.3$  & $1800$ \\			
                Amoeba-B \cite{Real18Regularized} & $2.55$ & $2.8$  & $3150$ \\
                PDARTS \cite{chen2019progressive} & $2.50$ & $3.4$ & $0.3$ \\      
                NAONet \cite{NAO} & $2.11$ & $128$ & $200$ \\  
                ProxylessNAS \cite{cai2018proxylessnas} & $2.08$ & $5.7$ & 10 \\  
    			ASAP + ET \cite{noy2019asap} & $1.94$ & $3.7$ & $0.2$ \\
                SharpDarts \cite{hundt2019sharpdarts} & $1.93$ & $3.6$ & $0.8$ \\       
                \hline
                XNAS-Small & $\bf{1.81}$ & $3.7$ & $0.3$ \\
                XNAS-Medium & $\bf{1.73}$ & $5.6$ & $0.3$ \\
                XNAS-Large & $\bf{1.60}$ & $7.2$ & $0.3$ \\

            \hline
            \end{tabular}
            \hspace{0.5pt}
            \captionof{table}{Classification errors of XNAS compared to state-of-the-art methods on CIFAR-10. The Search cost is measured in GPU days. Test error refers to top-1 test error (\%).\\ XNAS Small, Medium and Large refers to network architectures with XNAS cell and $36$, $44$ and $50$ initial channels respectively.}
            \label{cifar-10-results}
    \end{minipage} 
    \qquad
    \begin{minipage}[b]{.45\linewidth}
            % \centering                
            % \includegraphics[width=0.9\linewidth, height=95pt]{advantages_of_the_proposed_method/pics/normalized_entropy_vs_wd.png}
            % \captionof{figure}{Mean normalized entropy vs weight decay. The red dot refers to DARTS' settings.}
            % % \captionof{figure}{The mean normalized entropy across all the forecasters of a normal cell at the last search step $T$. The red dot refers to the official settings of DARTS.}
            % \label{fig:entropy_vs_wd}
            \begin{tabular}[t]{|l|c|c|c|}
            \hline
            \vtop{\hbox{\strut \textbf{ImageNet}}\hbox{\strut Architecture}}
                & \multicolumn{1}{|p{0.8cm}}{\centering Test\\error }
                & \multicolumn{1}{|p{0.9cm}}{\centering Params\\(M) }            
                & \multicolumn{1}{|p{0.8cm}|}{\centering Search\\cost}\\
                \hline
                SNAS \cite{snas}  & $27.3$ & $4.3$ & $1.5$\\ 
                ASAP \cite{noy2019asap}  & $26.7$ & $5.1$ & $0.2$\\
                DARTS \cite{liu2018darts} 
                & $26.7$ & $4.9$
                & $1$\\
                % PARSEC \cite{casale2019probabilistic} & $26.0$ & $5.6$ & 1\\
                NASNet-A \cite{NASNET} & $26.0$ & $5.3$ & $1800$\\
                PNAS \cite{PNAS}  & $25.8$ & $5.1$ & $150$\\   
                Amoeba-A \cite{Real18Regularized}  &  $25.5$ & $5.1$ & $3150$\\
                RandWire \cite{xie2019exploring} & $25.3$ & $5.6$ & $0$ \\
                SharpDarts \cite{hundt2019sharpdarts} & $25.1$ & $4.9$ & $0.8$ \\    
                Amoeba-C \cite{Real18Regularized}  &  $\bf{24.3}$ & $6.4$ & $3150$\\
                \hline
                XNAS & $24.6$ & $5.2$ & 0.3\\
                
                \hline
                \end{tabular}
                \hspace{0.5pt}
            \captionof{table}{Transferability classification error of XNAS, compared to top NAS cells, on ImageNet. Test error refers to top-1 test error (\%). Search cost is measured in GPU days.}
            \label{imagenet-results}
    \end{minipage}
\end{table}

==> related_work/differentiable_architecture_search.tex <==
\label{sec:differentiable_architecture_search}
In DARTS \cite{liu2018darts} an architecture is built from \emph{cells} represented as a directed acyclic graph, consisting of an ordered sequence of nodes. Every node $x_i$ is a feature map and each directed edge $(i, j)$ is associated with some operation $o^{(i,j)}$ that transforms $x_i$. Intermediate nodes are computed based on all of their predecessors:
\begin{equation}
   x^{(i)} =\sum_{j<i}o^{(i,j)}\left(x^{(j)}\right)
\end{equation}
In the search phase, every operation $o^{(i,j)}$ is replaced by a building block called \emph{Mixed Operations}:
\begin{equation}\label{eq:mixedOp}
\bar{o}_{i,j}(x)=\frac{\sum_{o\in\mathcal{O}}exp(\alpha_o^{(i,j)})o(x)}{\sum_{o'\in\mathcal{O}}exp(\alpha_{o'}^{(i,j)})}
\end{equation}
Each of which receives an input $x$, drives it through several candidate operations $o\in\mathcal{O}$ (e.g. convolution, max pooling, zero) and combines their outputs together into an output feature map $\bar{o}_{i,j}$. 
The set of parameters $w$ of all operations is denoted by $w$.
The combination is computed as a weighted average of the inner operations' outputs, with learned architecture weights $\alpha=\{\alpha_o^{(i,j)}\}$.
The architecture weights $\alpha$ and the operations' weights $w$ are learned jointly by alternately optimizing the validation loss $\nabla_\alpha\mathcal{L}_{val}(w,\alpha)$ and training loss $\nabla_w\mathcal{L}_{train}(w,\alpha)$, using gradient descent. 
At the end of the search, a discrete child architecture is obtained by replacing each mixed operation $\bar{o}^{(i,j)}$ by the most dominant operation: $o^{(i,j)} = \argmax_{o\in\mathcal{O}} \alpha_o^{(i,j)}$.


Due to the pervasive non-linearity in neural operations, the performance of the child network is always inconsistent and parameter retraining comes up as necessary.
To mitigate this bias, instead of taking the analytical expectation over the candidate operations, i.e. the mixed operation, SNAS \cite{xie2018snas} suggests to sample one operation in each mixed operation at every gradient descent step according to a learned joint distribution. This is done while preserving the differentialbilty of the NAS pipline. The authors show that their algorithm effectively performs a \emph{policy gradient search} \cite{williams1992simple}, with the reward associated with choosing the candidate operation j in the mixed operation i is equivalent to,
\begin{equation}
    R^{(i,j)}=-\nabla_{x^{(i)}}\mathcal{L}_{val} \cdot \bar{o}^{(i,j)}(x^{(j)}) \label{eq:reward}
\end{equation}
Our proposed EGW algorithm \ref{alg:EGW}, actually introduces an equivalent term in its update step.
% $-\nabla_{p_t}\ell (p_t,y_t)\cdot f_{t,i}$. 
% In some way, in this work, \ref{alg:EXGD} mitigates the sample inefficiency incurred for the sake of removing the bias, by optimizing the architecture $\alpha$ with respect to this same effective rewards, while avoiding the need of sampling.

% \nadav{I would remove the 'always' and write: "the performance of the child network is always inconsistent" => "the performance of the child network is inconsistent and model retraining is necessary."}

==> related_work/learning_from_experts/exponentiated_gradient_algo.tex <==
\begin{algorithm}[H] 
\caption{Exponentiated Gradient (EG)} 
\label{alg:EG}
\begin{algorithmic}[1]
\STATE \textbf{Input}: 
experts predictions $\left\{f_{t,i}\right\}_{i=0}^N ~ \forall t=1,\dots,T$,
\\  ~~~~~~~~~~~  step size $\eta$
\STATE \textbf{Init}: $w_{0,i} = 1 \quad\forall i=1,..,N$
\FOR{$t=1,..,T$}
\STATE $p_t=\frac{\sum_{i=1}^N w_{t-1,i} \cdot f_{t-1,i}}{\sum_{i=1}^N w_{t-1,i}}$ \label{eq:EG_prediction}
\STATE The loss gradient is revealed: $\nabla\ell (p_t,y_t)$
\STATE $w_{t,i} = w_{t-1,i}\cdot \exp{\{-\eta \nabla \ell (p_t,y_t) \cdot f_{t,i}\}}$ \label{eq:EG_update_rule}
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> related_work/learning_from_experts/learning_from_experts.tex <==
\label{sec:learning_from_experts}
Learning from experts \cite{cesa2006prediction} refers to a sequential decision making framework, dealing with a decision maker, i.e. a forecaster, whose goal is to predict an unknown outcome sequence $\{y_t\}_{t=1}^T \in \mathcal{Y}$ while having access to a set of N experts' advises, i.e. predictions. Denote these predictions at time $t=1,\dots,T$ by $f_{t,1},\dots, f_{t,N}\in \mathcal{D}$, where $\mathcal{D}$ is the \emph{decision space}, which we assume to be a convex subset of a vector space. Denote the forecaster's prediction $\{p_t\}_{t=1}^T \in \mathcal{D}$. Fix a non-negative loss function $\ell:\mathcal{D}\times\mathcal{Y}\xrightarrow{}\R$, which is convex in its first argument. At each time step $t=1,\dots,T$, the forecaster observes $f_{t,1},\dots, f_{t,N}$ and predicts $p_t$. The forecaster suffers $\ell(p_t , y_t)$ and the experts suffer $\ell(f_{t,i}, y_t)$. 
Denote the cumulative loss of the forecaster and of the expert i by,
\begin{align*}
 L_t=\sum_{s=1}^{t}\ell(p_s, y_s) \quad ; \quad  L_{t,i} = \sum_{s=1}^t \ell(f_{i,s}, y_s)
\end{align*} 
respectively. The goal of the forecaster is to minimize the regret, 
\begin{equation}\label{eq:experts_regret}
    R_T = L_T-\min_{i=1,\dots N}L_{t,i}
\end{equation}
\asaf{consider define regret with simplex-max to enhance the toy example}
In section \ref{sec:darts_as_learning_from_experts} we model the problem of differentiable architecture search of section \ref{sec:differentiable_architecture_search} as an experts problem. Here we present the main algorithm we build upon.
% One standing out algorithm is the \emph{Weighted Majority} (\ref{alg:WM}), \input{related_work/learning_from_experts/weighted_majority_algo.tex}
% with an appealing regret bound \cite{littlestone1994weighted}, 
% \begin{equation}
%     R_T\leq \sqrt{2T\log N} \quad\text{setting}\quad \eta = \sqrt{2\log N/T}
% \end{equation}
The \emph{Exponentiated Gradient} (EG) algorithm \ref{alg:EG} \cite{kivinen1997exponentiated} is a form of Follow-The-Regularized-Leader (FTRL) meta-algorithm \cite{kalai2005efficient} with an entropic regularizer. It effectively replaces the loss terms in the \emph{Weighted Majority} (WM) algorithm \cite{littlestone1994weighted} ($l_t(f_{t,i}, y_t))$ by the gradient of the loss projected on the expert's advice, i.e. %$l_t'(f_{t,i}) = \nabla_{p_t}\ell (p_t,y_t)\cdot f_{t,i}$ which we refer to as the \emph{loss proxy}.
\begin{equation}
    l_t'(f_{t,i}) = \nabla_{p_t}\ell (p_t,y_t)\cdot f_{t,i} \label{eq:loss_proxy}
\end{equation}
\input{related_work/learning_from_experts/exponentiated_gradient_algo.tex}
We are interested in gradient-based methods rather than loss based methods, since we deal with gradient-based NAS, see section \ref{sec:differentiable_architecture_search}, where gradients are derived through the back-propagation algorithm \cite{rumelhart1985learning}, as no explicit losses are associated with each decision variable, see \ref{sec:backprob_as_eg} for more details.
This proxy of the loss makes sense since, as stated in \cite{cesa2006prediction}: "This inner product is large if expert i’s advice $f_{t,i}$ points in the direction of the largest increase of the loss function. Such a large value means that having assigned a little bit larger weight to this expert would have increased the loss suffered at time t".
Moreover, for convex loss functions, a local linear approximation can only overestimate the regret, as stated in \cite{cohen16}, and used in corollary 2.5 of \cite{cesa2006prediction}. Furthermore, in section \ref{sec:backprob_as_eg} we connect between \eqref{eq:reward} and \eqref{eq:loss_proxy}, thus showing an equivalence to policy gradient search.
In \cite{cesa1999analysis} regret bounds are provided for the EG algorithm \ref{alg:EG}, when $\norm{\nabla\ell} \leq \mathbf{L}$ with experts' predictions within a convex subset of the euclidean unit ball, i.e. $\norm{f_{t,i}}\leq 1\,\forall t=1,\dots,T;\,i=1,\dots,N$:
\begin{equation}\label{eq:regret_bound}
    R_T\leq \mathbf{L}\sqrt{2T\log N} \quad\text{setting}\quad \eta = \frac{1}{\mathbf{L}}\sqrt{\frac{2\log N}{T}}
\end{equation}


==> related_work/learning_from_experts/weighted_majority_algo.tex <==
\begin{algorithm}[H] 
\caption{Weighted Majority (WM)} 
\label{alg:WM}
\begin{algorithmic}[1]
\STATE \textbf{Input}: 
experts predictions $\left\{f_{t,i}\right\}_{i=0}^N ~ \forall t=1,\dots,T$,
\\  ~~~~~~~~~~~  step size $\eta$
\STATE \textbf{Init}: $w_{0,i} = 1 \quad\forall i=1,..,N$
\FOR{$t=1,..,T$}
\STATE $p_t=\frac{\sum_{i=1}^N w_{t-1,i} \cdot f_{t-1,i}}{\sum_{i=1}^N w_{t-1,i}}$ \label{eq:WM_prediction}
\STATE \{Losses are revealed: $ \ell (f_{t,i},y_t)\ \quad\forall i=1,..,N$\}.
\STATE $w_{t,i} = w_{t-1,i}\cdot \exp{\{-\eta \ell (f_{t,i},y_t)\}}$ \label{eq:WM_update_rule}
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> related_work/related_work.tex <==
\subsection{Differentiable Architecture Search}
% Talk about DARTS -> Bias -> SNAS -> unbias
\input{related_work/differentiable_architecture_search.tex}

\subsection{Learning from Experts}
% Experts setup -> WM -> EG
\input{related_work/learning_from_experts/learning_from_experts.tex}


